Certified Defenses for Data Poisoning Attacks

Machine learning systems trained on user-provided data are susceptible to data poisoning attacks, whereby malicious users inject false training data with the aim of corrupting the learned model. While recent work has proposed a number of attacks and defenses, little is understood about the worst-case loss of a defense in the face of a determined attacker. We address this by constructing approximate upper bounds on the loss across a broad family of attacks, for defenders that first perform outlier removal followed by empirical risk minimization. Our approximation relies on two assumptions: (1) that the dataset is large enough for statistical concentration between train and test error to hold, and (2) that outliers within the clean (non-poisoned) data do not have a strong effect on the model. Our bound comes paired with a candidate attack that often nearly matches the upper bound, giving us a powerful tool for quickly assessing defenses on a given dataset. Empirically, we find that even under a simple defense, the MNIST-1-7 and Dogfish datasets are resilient to attack, while in contrast the IMDB sentiment dataset can be driven from 12% to 23% test error by adding only 3% poisoned data.

==> analysis.tex <==
\section{Further Analysis}
\label{sec:analysis}


==> defense.tex <==
\section{Defense Strategies}
\label{sec:defenses}
\label{sec:defense}
% go over the defenses

In this section we describe the defenses we consider, 
which range from basic ML best practices, to sophisticated 
anomaly detection techniques, to heuristics that we found 
useful when trying to defeat our constructed attacks. 

\todo{Pang-Wei fill the rest in}

\subsection{Certificates Against Worst-Case Attacks}
\label{sec:upper-bound}

For some of the defenses described above, we can derive 
\emph{worst-case certificates} showing that no possible 
poisoned dataset $\sD_p$ can cause the error to go above 
some threshold. These certificates are computed based on 
the clean data $\sD_c$. Importantly, they can \emph{not} 
be used in practice to achieve security guarantees (since 
the clean data is not available), but they are a helpful 
tool for benchmarking the performance of a defense strategy 
in cases where the clean data is known.

\todo{Pang-Wei fill the rest in}


==> experiments.tex <==
\section{Experiments}
\label{sec:experiments}

Recall our goal: to understand what properties of a dataset render 
it vulnerable or invulnerable against data poisoning attacks, and 
what sorts of defense strategies are most effective. At the same time, 
we would like to understand to what extent data poisoning may be an 
issue in practice, and how much resources a defender likely needs in 
order to be adequately robust.

% go over datasets
For our investigation, we considered a number of text and image classification 
datasets. \todo{describe datasets}

% for each dataset, 
For each dataset, we considered various subsets of the defenses 
from Section~\ref{sec:defense}. These were:
\begin{itemize}
\item TODO: go over defense strategies in a list and give them names (for reference in figures)
\end{itemize}
To evaluate these defense strategies, we deployed various attacks, described below. 
In addition, we derived worst-case certificates for the strategies [insert name here] using the 
upper bounding technique from Section~\ref{sec:upper-bound}. In our figures, we refer to 
these upper bounds as [insert name here].

For our attacks, \todo{descibe attacks}.

\todo{include figures, and interpretation}

% experiments

% interpretation



==> intuition.tex <==
\section{Intuition: Thwarting Defenses in High Dimensions}
% intuition: why attacks should be possible in high dimensions

Having described a number of defense strategies, we next give some intuition 
for why many, if not all, of these strategies can perform poorly in high dimensions.

% describe simple Gaussian dataset (include figure)
To do this, we consider a simple Gaussian dataset in $\bR^d$. Let $e_1$ be the unit vector 
pointing in the direction $(1,0,0,\ldots)$; for some scalar $\lambda > 0$, 
the points in the positive class are drawn from a Gaussian $\sN(\lambda e_1, I)$, while the 
points in the negative class are drawn from $\sN(-\lambda e_1, I)$. 

It is easy to see that the optimal classifier is $f(x) = \sign(e_1^{\top}x) = \sign(x_1)$. 
The disribution of $x_1$ under the positive class is $\sN(\lambda, 1)$, and under the 
negative class is $\sN(-\lambda, 1)$, so the two classes are well-separated as long as 
$\lambda \gg 1$. For instance, if $\lambda = 2$ then the classifier $f$ achieves error 
less than $2.3\%$.
% TODO: want to include some sort of figure, maybe show projection onto true direction, 
% and onto two random directions

% what can the poisoner do? add data along line between means, distance \sqrt{d}
What strategy can the attacker employ in this setting? We first make the following 
(perhaps unintuitive) observation: despite the fact that the classes are well-separated, 
the average distance from a point to its class mean is roughly $\sqrt{d}$, while the distance 
between class means is only $2\lambda = 4$. In particular, the point $-(\sqrt{d}-\lambda)e_1$ 
is no further away from the center of the positive class than is typical, but would have an 
inordinate impact on the learned classifier.

Therefore, the attacker will employ the following strategy: place $\frac{1}{2}\epsilon N$ 
positive points at $x_p^+ = -(\sqrt{d}-\lambda)e_1$, and $\frac{1}{2}\epsilon N$ negative 
points at $x_p^- = (\sqrt{d}-\lambda)e_1$. This poisoned data is enough to completely flip 
the direction of the learned classifier provided that $\epsilon > ???$.

% points don't look any further away than other points, yet together create large influence

% emphasize this is a (possibly unintuitive) phenomenon

% how much data needed to completely flip learned model?

% shows that no anomaly detector algorithm (that just looks at individual points) can work, 
%   need to somehow consider points as a population and identify directions of large 
%   deviation (cite relevant papers)


==> results-dogfish-figure.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=0.32\textwidth]{figures/fig1-dogfish.pdf}
\includegraphics[width=0.32\textwidth]{figures/fig2-dogfish.pdf}
\includegraphics[width=0.32\textwidth]{figures/fig3-dogfish.pdf}
\end{center}
\caption{The same experiments as in Figure~\ref{fig:results-mnist}, reported 
on the Dogfish dataset.}
\label{fig:results-dogfish}
\end{figure}

